Multi-objective Electric Vehicle Charging Strategies at Energy Hubs with Justice-informed Profit Distribution among Users

This paper studies potential energy cost savings in electric vehicle (EV) charging hubs when users allow cooperative vehicle-to-grid (V2G), and how such savings should be redistributed. To this end, we present multi-objective operational strategies and justice-informed profit sharing methods for a charging energy hub equipped with a battery storage system and solar panels. Specifically, we first frame the dynamic energy hub operational problem aiming to minimize a combination of grid costs and emissions, accounting for time-varying prices and energy mix as well as storage system and EV battery degradation, which is especially relevant when considering V2G operations. We parse the problem as a second-order conic program that can be efficiently solved to global optimality. Our real-world case-study shows the importance of flexibility for hub operation: Equipping a charging station with a stationary battery and leveraging dynamic V2G can significantly reduce the total costs and emissions compared to conventional settings without a battery or dynamic charging by more than 10%. To redistribute these cost benefits to users, we compare standard Nash bargaining with a justice-informed sufficientarian version which caps charging prices to safeguard adequate access to affordable charging. Our results show that the sufficientarian approach better accounts for inequalities in flexibility capital without significantly affecting aggregate costs, highlighting how justice-informed pricing only marginally affects total revenues.

==> Chapters/Case_Study_fairness.tex <==
\section{Case study fair cost distribution}
\label{Ch:Case_study_fairness}

% beta is 10% (profit margin)

In order to compare the different distributions we apply them to a case study. For this case study we use a different EV charging demand dataset. In this case study the EV charging demand comes from charging stations for cars at the Caltech campus in California, USA~\cite{}. This data is subsequently shifted from California time to Dutch time just like with the PV energy generation data For the PV generation data and the energy cost and emissions we take the same sources as for the case study in Chapter~\ref{ch:Case_study}. However, since the total energy demand throughout a year is significantly less, the average energy tax is higher. In this case study we use an average energy tax of $0.05548$~€/kWh~\cite{Belastingdienst2026}.

We also change the parameters to scale with the EV charging dataset. These parameters can be found in~\autoref{tab:Optimisation_parameters_fairness}. The charger and grid costs don't scale linearly with the size, especially since we chose to use low power chargers in this case study. Therefore, new parameters can be found in~\autoref{tab:Cost_parameters_fairness}. The parameters not present in \autoref{tab:Cost_parameters_fairness} are the same for both case studies and can be found in \autoref{tab:Cost_parameters}.

\begin{table}[]
\centering
\caption{Fairness case study parameters}
\label{tab:Optimisation_parameters_fairness}
\begin{tabular}{l|l|r|l}
Parameter                                   & Variable                   & Value & Unit \\ \hline
$E_{\mathrm{b}}^\mathrm{inst}$  & Total installed BESS capacity & 100 & kWh \\
$\overline{E}_{\mathrm{b}}$     & Max. useable BESS energy   & 90   & kWh  \\
$\underline{E}_{\mathrm{b}}$    & Min. useable BESS energy   & 10   & kWh  \\
$\overline{P}_{\mathrm{b}}$     & Max. BESS power            & 10   & kW   \\
$\underline{P}_{\mathrm{b}}$    & Min. BESS power            & -10  & kW   \\
$\overline{P}_{\mathrm{g}}$     & Max. grid power            & 100  & kW   \\
$\underline{P}_{\mathrm{g}}$    & Min. grid power            & -100 & kW   \\
$\overline{P}_{\mathrm{ch}, n}$ & Max. EV charging power     & 11   & kW   \\
$\underline{P}_{\mathrm{ch}, n}^{\mathrm{V2G}}$ & Max. EV discharge power & -11  & kW    \\
$\underline{P}_{\mathrm{ch}, n}^{\mathrm{V1G}}$ & Max. EV discharge power & 0  & kW  \\
\textbf{Datasets} &&\\
$P_{\mathrm{pv}}^\mathrm{inst}$ & Installed PV capacity & 21  & $\mathrm{kW_p}$  \\
& Average number of EVs & 29.1 & $\textrm{day}^{-1}$ \\
& Average EV connection time & 6.06 & h\\
& Average EV charging demand & 8.92 & kWh\\
\textbf{Optimisation} &&\\
$\Delta t$ & size of the timestep & 0.25 & h\\
$\alpha_r$ & regularisation weight & $2\cdot10^{-3}$ \\

\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{Case study cost parameters that changed wrt. \autoref{tab:Cost_parameters}}
\label{tab:Cost_parameters_fairness}
\begin{tabular}{l|r|l|l}
Parameter &  Value & Unit & Source \\ \hline

\textbf{Grid infrastructure} &&&\\
$\mathrm{CAPEX}_\mathrm{grid}^\text{€}$ & 70 & $\text{€}/\mathrm{kW}$ & \cite{TetteroVerdegaalEtAl2022} \\
$\mathrm{OPEX}_\mathrm{grid}^\text{€}$  & 27 & $\text{€}/\mathrm{kW}/\textrm{year}$ & \cite{TetteroVerdegaalEtAl2022} \\
$a_\mathrm{grid}^\text{€}$ & 3.0 & $\mathrm{ct}/\mathrm{kWh}$ & \eqref{eq:grid_amort_price} \\

\textbf{Chargers} &&&\\
$\mathrm{CAPEX}_\mathrm{chg}^\text{€}$ & 3000 & $\text{€}/\mathrm{charger}$ & \cite{TetteroVerdegaalEtAl2022,LanzNollEtAl2022} \\
$\mathrm{OPEX}_\mathrm{chg}^\text{€}$  & 100 & $\text{€}/\mathrm{charger}/\textrm{year}$ & \cite{TetteroVerdegaalEtAl2022,LanzNollEtAl2022} \\
$\mathrm{C}_\mathrm{chg}^\mathrm{GHG}$ & 622 & kg $\mathrm{CO_2e}/\mathrm{charger}$ & \cite{Dubois2024} \\
$N_\mathrm{chgs}$ & 10 & chargers & \\
$a_\mathrm{grid}^\text{€}$ & 12.6 & $\mathrm{ct}/\mathrm{kWh}$ & \eqref{eq:chargers_amort_price} \\
$a_\mathrm{chg}^\mathrm{GHG}$ &  & kg $\mathrm{CO_2e}/\mathrm{charger}/$ & \eqref{eq:chargers_amort_price} \\

\end{tabular}
\end{table}

For all calculations we average all data throughout a year by doing an optimisation for 24 different dates, 2 each month, with a window of 5 days for each starting date.

Before we can assess the fairness of different distributions we first need to determine what fair means. In our case we have a few properties that a fair distribution should fulfill:
\begin{enumerate}
    \item A user's charging price should decrease when their provided flexibility allows the system reduce the total system costs; % marginal contributions
    \item Users with limited flexibility should not receive disproportionate costs since these users are generally already worse off \cite{Libertson2022,MalabananSauriLavieriEtAl2025};
    % \item Users should be compensated for the increased battery degradation due to V2G participation; % Pareto optimality with battery degradation in the objective.
    % \item Both the station operator and the users who allow V2G should benefit from the value generated by V2G; % Pareto optimality (again)
    % \item Smart charging should leave both the charging station and all users better off than a baseline; % Pareto optimality
    % \item EVs with similar service requests and flexibility should have similar charging prices.% (Anonimity / consistency / symmetry axiom).
\end{enumerate}

\subsection{Disagreement outcome}
Both the Nash and Aumann-Shapley allocations depend on the disagreement outcome. We assume that in this disagreement case the users decide to not charge at our energy hub but at another charging station. 

% For the EV utility $u_{\mathrm{ev}, n}^\mathrm{d}$ we assume users decide to charge at a different charging station where they are charged according to the nominal charging
For the EVs this means that they will pay the price of a different charging station where they are charged according to nominal charging. We calculate the charging costs in the case of disagreement using
\begin{equation}
    \label{eq:disagreement_nominal}
    C_{\mathrm{ev}, n}^{\mathrm{d}} = \beta \cdot C_{\mathrm{ev}, n}^{\mathrm{nom}} = \beta\cdot\sum_{k=1}^{N_\mathrm{T}}p_{\mathrm{imp}, k} \cdot P_{\mathrm{ev}, k, n}^{\mathrm{nom}}\cdot \Delta t,
\end{equation}
where $C_{\mathrm{ev}, n}^{\mathrm{nom}}$ is the charging cost for EV $n$ in the case of nominal charging, $\beta$ is the different charging station's profit margin and $P_{\mathrm{ev}, k, n}^{\mathrm{nom}}$ is calculated using~\cref{eq:Nominal_strat}. We then calculate EV disagreement utitility ($u_{\mathrm{ev}, n}^\mathrm{d}$) using~\cref{eq:utility_ev}. We set $\beta=1.1$.

Given that all users decide to charge at a different station the charging station will not do any EV charging and have just the PV panels and BESS to generate a profit. The operator disagreement utility is found by solving Problem~\ref{prob:simple_optimisation} without any EVs. With the results of this optimisation without EVs we calculate the station operator disagreement utility ($u_{\mathrm{op}}^\mathrm{d}$) using~\cref{eq:utility_operator} where we do not have any income from EVs, thus $C_{\mathrm{ev}, n}^\mathrm{d} = 0$.



\subsection{Nash bargaining}
In the case of weighted Nash bargaining with the charged energy as weight, the result is an equal price decrease for all users, except for the users using V2G. In the case of V2G the extra battery degradation due to V2G is compansated and thus these users pay less for charging. This can be seen in \autoref{fig:Nash_price_change} where the price change with respect to the nominal price is shown. All sessions where normal smart charging (V1G) is done have the same price decrease. Only sessions where V2G is used, indicated with a star, have a larger decrease in charging price.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Ch_fairness_comp/Nash_price_imp_May.pdf}
    \caption{Charging price change wrt. nominal charging for all charging sessions in a 5 day period at the start of May for Nash bargaining. V1G charging is indicated with a circle, V2G charging with a star.}
    \label{fig:Nash_price_change}
\end{figure}


\subsection{Sufficientarian Nash bargaining}
We determine the upper limit of the charging price $\overline{p}_\mathrm{ev}$ by taking the 90th percentile of the Nash barginaining price of a random subset of sessions throughout a year as per Daniel's biostatistical approach to normal functioning~\cite{Martens2017}.

In \autoref{fig:Nash_price_starttime} the charging price for both Nash bargaining and sufficientarian Nash bargaining for all charging sessions in a 5 day window are shown depending on the arrival time. The upper limit in the sufficientarian Nash bargaining prevents users from paying too much. We can see that there are no sessions that have to pay more than the limit. For sessions below the limit the prices barely change, hence why the Nash prices are not all visible as the sufficientarian Nash prices are plotted on top.
However, we can also see that the users arriving in the middle of the day pay significantly less than users arriving early in the morning or in the evening. This highlights the disadvantage of the Nash approach, even though the price decrease is the same for all V1G users, the resulting price is highly dependent on the disagreement price.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Ch_fairness_comp/Nash-suff_comp_Feb.pdf}
    \caption{Charging prices for all charging sessions in a 5 day period in the middle of February for different distribution principles. V1G charging is indicated with a circle, V2G charging with a star. Along with the 5 day average grid electricity price and charger amortisation costs.}
    \label{fig:Nash_price_starttime}
\end{figure}

\subsection{Aumann-Shapley allocation}
For the numerical integration done in the Aumann-Shapley method we use the trapezoidal method with 100 integration steps, thus $\Delta\lambda = 0.01$.

\autoref{fig:AS_charging_price_starttime} shows the charging price determined through the Aumann-Shapley allocation. It can be seen that all charging sessions which are still connected in the middle of the day (when the electricity is cheapest) all have a low charging price. However, charging sessions connecting later in the afternoon and evening, which consequently are not able to charge at the lowest electricity prices, pay more. Therefore, with this distribution priciple we give disadvantaged users an even bigger disadvantage.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Ch_fairness_comp/AS_Feb.pdf}
    \caption{Charging prices for all charging sessions in a 5 day period in the middle of February for Aumann-Shapley allocation. V1G charging is indicated with a circle, V2G charging with a star. Along with the 5 day average grid electricity price and charger amortisation costs.}
    \label{fig:AS_charging_price_starttime}
\end{figure}

What we can see though, is that EVs staying for similar amounts of time and therefore, EVs for which the actual charging is scheduled at the same time, have similar charging prices. 



\subsection{Comparison}

% Adding the limit in sufficientarian does not significantly change the average

In \autoref{tab:prices_averaged} the average charging prices and average station profits throughout a year are shown. These prices are determined by doing the calculations for 24 windows of 5 days throughout the year, 2 for each month. The averages for all allocations are very similar. However, there are differences in how these prices are distributed among the users. 
The histogram in \autoref{fig:Histograms_S_Nash-AS} shows the distribution of charging prices throughout a year for the sufficientarian Nash and AS allocation. This shows that the sufficientarian Nash distribution makes sure that no user pays more than the set maximum. However, the AS allocation does have some users that pay more than the maximum. On the other hand, the AS allocation has less spread in the prices


\begin{table}[]
\centering
\caption{The prices for all considered allocation methods averaged over the year.}
\label{tab:prices_averaged}
\begin{tabular}{l|c|c}
Allocation method & Av. charging price & Av. station profits \\ \hline
Nominal charging & \texteuro 0.332 /kWh & \texteuro 31.7 \\
Nash bargaining & \texteuro 0.291 /kWh & \texteuro 88.6 \\
Sufficientarian Nash & \texteuro 0.290 /kWh & \texteuro 86.6 \\
AS allocation & \texteuro 0.291 /kWh & \texteuro 88.1
\end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Ch_fairness_comp/Hist_comp_S_Nash-AS_year.pdf}
    \caption{Histograms of the charging prices throughout a year for the sufficientarian Nash and AS allocation.}
    \label{fig:Histograms_S_Nash-AS}
\end{figure}


\subsubsection*{1) Users should be incentivised to charge at advantageous times}
In order to determine this we take a look at all vehicles arriving before 9 in the morning, before the electricity price drops later in the day. We then look at how the price changes depending on the amount of time a user stays connected. If this requirement is fulfilled we would expect users that stay connected for only a few hours to have to pay more than users that stay connected the whole day and who are subsequently able to charge at the cheap times in the middle of the day.
\autoref{fig:morning-connection_time} shows the prices for all sessions starting before 9 in the morning for 5 days in July for sufficientarian Nash and AS allocation. What we can see is that for sufficientarian Nash all have to pay a similar price, independent of how long they are connected (ignoring the two outliers). While for AS the users who stay connected to the station longer and thus provide more flexibility generally have to pay less.

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Ch_fairness_comp/morning_Tch_Jul.pdf}
    \caption{Charging prices for all sessions starting before 9 in the morning for a window of 5 days in the middle of July depending on the total connection time. V1G charging is indicated with a circle, V2G charging with a star.}
    \label{fig:morning-connection_time}
\end{figure}

\subsubsection*{2) Users without flexibility should not be disadvantaged by having higher charging prices}

In the case of sufficientarian Nash we used an upper limit on the charging price to make sure none of the users has to pay too much for charging. Such a limit is not implemented in the AS allocation. Additionally, rewarding flexibility is inherent to the AS approach. It determines the charging price depending on the marginal contribution of each user. Therefore, if a user does not have any flexibility to charge at opportune times they will receive almost none of the profit. For AS allocation flexibility is directly rewarded but the flip side of this is that inflexibility is directly punished.
 
% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{Figures/Ch_fairness_comp/AS-suff_Nash_comp_Feb.pdf}
%     \caption{Charging prices for all charging sessions in a 5 day period in the middle of February for sufficientarian Nash and Aumann-Shapley allocation. V1G charging is indicated with a circle, V2G charging with a star. Along with the 5 day average grid electricity price and charger amortisation costs.}
%     \label{fig:AS-Suff_Nash_comp_feb}
% \end{figure}



\subsubsection*{3) Users should not be penalised for allowing V2G in the form of increased battery degradation}

% (Sufficientarian) Nash does this through (33) (and subsequently 36,37) while AS does this through (51)

\subsubsection*{4) There should be an incentive for both the station operator and the users to use V2G}

% for (sufficientarian) Nash this is not necessarily the case. V2G profits are distributed over all agents and therefore the user that enables V2G only sees a small fraction of the profits. 
% For AS the agent that enables V2G is directly compensated for the profits generated through V2G (inherent to the AS approach). Then, through the 50% sharing with the station it only gets 50% of the profits from V2G

\subsubsection*{5) Smart charging should be advantageous for both the charging station and the users}
For the Nash and the sufficientarian Nash this requirement is baked in in the form of the constraints in \cref{eq:constr_util_ev,eq:constr_util_op}, the utilities for the users and the station operator have to improve, otherwise the disagreement option will be chosen and no smart charging will be done.

For the AS allocation this is not guaranteed, especially for users arriving at the cheapest time, when nominal charging would also be cheap. In such a case it could occur that the marginal cost determined with AS allocation is higher than the nominal charging price.


\subsubsection*{6) EVs with similar requests should have similar charging prices}






==> Figures/Ch_energy_hub_model/Charging_strats.tex <==
%% Creator: Inkscape 1.1 (c68e22c387, 2021-05-23), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'Charging_strats.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{367.33216925bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,1.15188502)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength]{Figures/Ch_energy_hub_model/Charging_strats_NOTEXT.pdf}}%
    \put(0.93,0.521){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\Large t\end{tabular}}}}%
    \put(0.85,0.54){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$t_\mathrm{f}$\end{tabular}}}}%
    \put(0.18,0.54){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$t_\mathrm{s}$\end{tabular}}}}%
    \put(-0.01,1.06){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}\Large $P_\mathrm{ev}$\end{tabular}}}}%
    \put(0,0.981){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\overline{P}_\mathrm{ev}$\end{tabular}}}}%
    \put(0,0.565){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\underline{P}_\mathrm{ev}$\end{tabular}}}}%
    \put(0,0.148){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$\underline{P}_\mathrm{ev}$\end{tabular}}}}%
  \end{picture}%
\endgroup%


==> Figures/Ch_energy_hub_model/power_per_EV4.tex <==
%% Creator: Inkscape 1.1 (c68e22c387, 2021-05-23), www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'power per EV4.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{785.99506875bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.74405599)%0.67405599
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0.005){\includegraphics[width=\unitlength,page=1]{Figures/Ch_energy_hub_model/power per EV4.pdf}}%
    \put(0.87,0.37){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Time\end{tabular}}}}%
    \put(0.87,0.0){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}Time\end{tabular}}}}%
    \put(0.02,0.53){\rotatebox{90}{\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}EV power\end{tabular}}}}}%
    \put(0.02,0.16){\rotatebox{90}{\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}EV power\end{tabular}}}}}%
    \put(0.89,0.692){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$P_{\mathrm{ev},1}$\end{tabular}}}}%
    \put(0.89,0.645){\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$P_{\mathrm{ev},2}$\end{tabular}}}}%
  \end{picture}%
\endgroup%

